LLMPirate: LLMs for Black-box Hardware IP Piracy

The rapid advancement of large language models (LLMs) has enabled the ability to effectively analyze and generate code nearly instantaneously, resulting in their widespread adoption in software development. Following this advancement, researchers and companies have begun integrating LLMs across the hardware design and verification process. However, these highly potent LLMs can also induce new attack scenarios upon security vulnerabilities across the hardware development process. One such attack vector that has not been explored is intellectual property (IP) piracy. Given that this attack can manifest as rewriting hardware designs to evade piracy detection, it is essential to thoroughly evaluate LLM capabilities in performing this task and assess the mitigation abilities of current IP piracy detection tools. Therefore, in this work, we propose LLMPirate, the first LLM-based technique able to generate pirated variations of circuit designs that successfully evade detection across multiple state-of-the-art piracy detection tools. We devise three solutions to overcome challenges related to integration of LLMs for hardware circuit designs, scalability to large circuits, and effectiveness, resulting in an end-to-end automated, efficient, and practical formulation. We perform an extensive experimental evaluation of LLMPirate using eight LLMs of varying sizes and capabilities and assess their performance in pirating various circuit designs against four state-of-the-art, widely-used piracy detection tools. Our experiments demonstrate that LLMPirate is able to consistently evade detection on 100% of tested circuits across every detection tool. Additionally, we showcase the ramifications of LLMPirate using case studies on IBEX and MOR1KX processors and a GPS module, that we successfully pirate. We envision that our work motivates and fosters the development of better IP piracy detection tools.

==> Sec4_pirating_soft_ips.tex <==
\subsection{LLMs for Pirating Soft IPs}
LLMs such as OpenAI's GPT-3.5 and GPT-4 are trained on vast amounts of data from various sources, such as CommonCrawl \textcolor{blue}{Note: To me, CommonCrawl seems less recognizable than the other sources - I could be wrong. Maybe could be a more general description of it}, Wikipedia, books, synthetic data, and even code repositories such as GitHub, which contain software and hardware codes~\cite{}. 
% Since these LLMs are tr which also contain programming languages. 
\textcolor{blue}{As} %Since%
these LLMs are trained on programming languages, they learn to understand, generate, and even rewrite codes in hardware description languages (HDLs) such as Verilog and VHDL, just like natural languages such as English and French. 
Since most of the HDL codes implementing IPs in the LLM training data is at the RTL abstraction (as opposed to a gate-level netlist abstraction), here we attempt to pirate soft IPs, i.e., IPs in the form of RTL code. More specifically, 
we prompted GPT-3.5 
\textcolor{blue}{(chosen due to its state-of-the-art capability~\cite{})} to rewrite a Verilog RTL code for a 4-bit adder circuit.
\textcolor{blue}{This circuit is chosen due to adders being} one of the most fundamental components in virtually all modern computing systems. The objective here is to check the LLM's ability to rewrite the soft IP, i.e., the RTL code of the circuit, so that it is not flagged by IP piracy detection tools but still maintains the same functionality. Listings~\ref{listing:4_bit_adder_rewriting_prompt} and~\ref{listing:4_bit_adder_rewriting_response} illustrate our prompt and the response generated by GPT-3.5, respectively. It is clear that not only does GPT-3.5 understand that the provided Verilog RTL code is for a 4-bit adder (apparent by its definition of the \texttt{adder} submodule on line 24), it successfully generates a functionally-equivalent 4-bit adder RTL code using a different structure
(by separating the addition logic into a separate submodule), as requested.


\lstinputlisting[language=Verilog, label = {listing:4_bit_adder_rewriting_prompt}, caption={Prompt to GPT-3.5 for rewriting Verilog RTL}, style=prettyverilog, float, belowskip=-5pt, aboveskip=20pt, firstnumber=1, linewidth=\linewidth]{4-bit_adder_rewriting_prompt.v}

\lstinputlisting[language=Verilog, label = {listing:4_bit_adder_rewriting_response}, caption={GPT-3.5's response to the prompt in Listing~\ref{listing:4_bit_adder_rewriting_prompt}}, style=prettyverilog, float, belowskip=-5pt, aboveskip=20pt, firstnumber=1, linewidth=\linewidth]{4-bit_adder_rewriting_response_new.v}


\noindent\textbf{Limitations.} Although the above example illustrates that GPT-3.5 successfully generates a structurally-different functionally-equivalent code for the relatively simple adder module, when we evaluate this rewritten code for piracy using GNN4IP (the state-of-the-art hardware IP piracy detection tool), GNN4IP flags it as pirated from the original code. This observation holds true for other simple codes too. Moreover, for more complicated codes such as the Rule90 cellular automaton from HDLBits~\cite{HDLBits_Rule90}, GPT-3.5 struggles to generate even functionally-equivalent RTL code (see Listings~\ref{listing:rule_90_rewriting_prompt} and~\ref{listing:rule_90_ChatGPT_incorrect_response} in Sec.~\ref{sec:GPT3_5_struggle} in the Appendix). Such observations also hold true for other LLMs, such as GPT-4 and CoPilot. Thus, off-the-shelf LLMs are not capable of pirating soft IPs, i.e., RTL codes, because either (i) the rewritten codes are similar to the original codes and hence \textbf{flagged by IP piracy detection tools}, or worse, (ii) the rewritten codes are \textbf{not functionally equivalent} to the original codes. To address these limitations and successfully pirate hardware IPs, %next,% 
we \textcolor{blue}{then} devise a formulation to pirate firm IPs, i.e., gate-level netlists, using LLMs.

==> authors.tex <==
\author{Vasudev Gohil}
\affiliation{%
  \institution{Texas A\&M University}
  \city{College Station}
  \state{Texas}
  \country{United States}
  }
\email{gohil.vasudev@tamu.edu}

\author{Matthew DeLorenzo}
\affiliation{%
  \institution{Texas A\&M University}
  \city{College Station}
  \state{Texas}
  \country{United States}
  }
\email{matthewdelorenzo@tamu.edu}

\author{Veera Vishwa Achuta Sai Venkat Nallam}
\affiliation{%
  \institution{Texas A\&M University}
  \city{College Station}
  \state{Texas}
  \country{United States}
  }
\email{nallamsaiv@tamu.edu}

\author{Joey See}
\affiliation{%
  \institution{Texas A\&M University}
  \city{College Station}
  \state{Texas}
  \country{United States}
  }
\email{joeysee@tamu.edu}

\author{Jeyavijayan Rajendran}
\affiliation{%
  \institution{Texas A\&M University}
  \city{College Station}
  \state{Texas}
  \country{United States}
  }
\email{jv.rajendran@tamu.edu}


% \author{Vasudev Gohil, Matthew DeLorenzo, Veera Vishwa Achuta Sai Venkat Nallam, \\Joey See, Jeyavijayan Rajendran\\
% Texas A\&M University, USA\\
% {\tt \{gohil.vasudev, matthewdelorenzo, nallamsaiv, joeysee, jv.rajendran\}@tamu.edu}}
